Fast Feedback Control over Multi-hop Wireless Networks with Mode Changes and Stability Guarantees

Closing feedback loops fast and over long distances is key to emerging cyber-physical applications; for example, robot motion control and swarm coordination require update intervals of tens of milliseconds. Low-power wireless communication technology is preferred for its low cost, small form factor, and flexibility, especially if the devices support multi-hop communication. Thus far, however, feedback control over multi-hop low-power wireless networks has only been demonstrated for update intervals on the order of seconds. To fill this gap, this paper presents a wireless embedded system that supports dynamic mode changes and tames imperfections impairing control performance (e.g., jitter and message loss), and a control design that exploits the essential properties of this system to provably guarantee closed-loop stability for physical processes with linear time-invariant dynamics in the presence of mode changes. Using experiments on a cyber-physical testbed with 20 wireless devices and multiple cart-pole systems, we are the first to demonstrate and evaluate feedback control and coordination with mode changes over multi-hop networks for update intervals of 20 to 50 milliseconds.

==> img/evalPendulum.tex <==
% !TEX root = ../paper.tex
\begin{figure}
\centering
%
\tikzsetnextfilename{cartPole}
\begin{tikzpicture}[scale=0.7, every node/.style={scale=0.7}]]
\tikzstyle{ground}=[fill,pattern=north east lines,draw=none,minimum width=5,minimum height=0.1]
\tikzset{>=latex};
\draw(0.5,0.35)rectangle(-0.5,-0.35);
\draw[fill=white](-0.25,-0.5)circle(0.2);
\draw[fill=white](0.25,-0.5)circle(0.2);
\draw[ultra thick,lightgray](0,0)node(cart){}--(1,2.5);
\draw[fill=black](1,2.5)circle(0.2)node(pole){};
\draw[dashed] (0,0.5) -- (0,2.5)node(top){};
\draw[fill=black](0,0)circle(0.05);
\draw[fill=black](-0.25,-0.5)circle(0.025);
\draw[fill=black](0.25,-0.5)circle(0.025);
\node[ground,minimum width=200,anchor=north](floor)at(0,-0.7){};
\draw(floor.north east)--(floor.north west);
 \draw pic[" ",draw=black, -,  angle eccentricity=1.5,angle radius =
  2cm] {angle = pole--cart--top};
\draw[->](-1.5,1.5)node[above]{Cart} -- (-0.6,0.25);
\draw[->] (2,1.5)node[right]{Pole} -- (1,2);
\draw[->]([shift={(0,-0.2cm)}]floor.south west) -- node[midway,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:0,fill=black]{}
node[pos=0.4,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:-5,fill=black]{}
node[pos=0.3,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:-10,fill=black]{}
node[pos=0.2,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:-15,fill=black]{}
node[pos=0.1,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:-20,fill=black]{}
node[pos=0,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:-25,fill=black]{}
node[pos=0.6,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:5,fill=black]{}
node[pos=0.7,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:10,fill=black]{}
node[pos=0.8,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:15,fill=black]{}
node[pos=0.9,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:20,fill=black]{}
node[pos=1,draw,rectangle,inner sep = 0, minimum width=0.1em, minimum height=0.4em,label=below:25,fill=black]{}
([shift={(0,-0.2cm)}]floor.south east);
\draw[->] (-3,0.5)node[above]{Track} -- ([shift={(-2.5,0.1cm)}]floor.north);
\node[below = 2.5em of floor,inner sep = 0]{Cart Position $s$ [\si{\centi\meter}]};
\draw[->](1,0.75)node[below right]{Pole Angle $\theta$ [\si{\degree}]} -- (0.25,1.5);
\end{tikzpicture}
\caption{Schematic of a cart-pole system.}
\label{fig:pendulum}
\end{figure}


==> img/glossy_time_sync_error.tex <==
% !TEX root = ../paper.tex
\begin{figure}[!tb]%[t]
	\centering
	\includegraphics[width=0.5\linewidth]{glossy_time_sync_error}
	\caption{Time synchronization error between~{\cp}s.}
	\label{fig:glossy_time_sync_error}
\end{figure}

